Detrimental Contexts in Open-Domain Question Answering

For knowledge intensive NLP tasks, it has been widely accepted that accessing more information is a contributing factor to improvements in the model's end-to-end performance. However, counter-intuitively, too much context can have a negative impact on the model when evaluated on common question answering (QA) datasets. In this paper, we analyze how passages can have a detrimental effect on retrieve-then-read architectures used in question answering. Our empirical evidence indicates that the current read architecture does not fully leverage the retrieved passages and significantly degrades its performance when using the whole passages compared to utilizing subsets of them. Our findings demonstrate that model accuracy can be improved by 10% on two popular QA datasets by filtering out detrimental passages. Additionally, these outcomes are attained by utilizing existing retrieval methods without further training or data. We further highlight the challenges associated with identifying the detrimental passages. First, even with the correct context, the model can make an incorrect prediction, posing a challenge in determining which passages are most influential. Second, evaluation typically considers lexical matching, which is not robust to variations of correct answers. Despite these limitations, our experimental results underscore the pivotal role of identifying and removing these detrimental passages for the context-efficient retrieve-then-read pipeline. Code and data are available at https://github.com/xfactlab/emnlp2023-damaging-retrieval

==> figures/3-method-plots.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{./img/attention-score-small.png}
  \caption{Attention score of top-10 retrieved passages. The attention score is highest for the 8th passage and the passage is neither \textbf{DP} nor \textbf{DN}}
  \label{fig:attention-score-small}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{./img/density-plot.png}
  \caption{Attention density plot of top-20 passages in NQ development set. \textbf{DP} contexts relatively present high attention score.}
  \label{fig:attention-density}
\end{figure}

==> figures/appen-1-2.tex <==
\begin{table}[h!]
\small
\centering
\begin{tabular}{@{}cc|ccccc@{}}
\toprule
Dataset                   & Retriever  & initial zeros     & definite positive & definite negative & semi positive        & semi negative     \\ 
\midrule
\multirow{3}{*}{NQ}       & DPR        & 17.2 (1338/24235) & 82.6 (5383/6513)   & 24.8 (475/1912)   & 13.1 (57894/440478)  & 10.2 (1077/72462) \\
                          & SEAL       & 19.7 (7769/39358) & 45.3 (2801/6178)  & 23.4 (434/1803)   & 13.3 (54066/406500)  & 11.8 (7885/66361) \\
                          & Contriever & 21.4 (7586/35289) & 45.4 (2951/6490)  & 24.8 (510/2052)   & 13.0 (54143/414398)  & 11.7 (8767/74871) \\ \midrule
\multirow{3}{*}{TriviaQA} & DPR        & 12.8 (2394/18639) & 78.3 (6068/7749)  & 23.0(312/1356)    & 23.5 (145712/617739) & 11.1 (4630/41517) \\
                          & SEAL       & 24.4 (8278/33835) & 55.0 (4031/7317)  & 26.3 (364/1379)   & 24.3 (135909/558537) & 13.9 (5382/38532) \\
                          & Contriever & 22.9 (6176/26861) & 55.6 (4259/7654)  & 26.7 (399/1490)   & 23.9 (140800/588172) & 13.0 (5603/43023) \\ \bottomrule
\end{tabular}
\caption{Percentage of passages including answers by contextual sections}
\end{table}

==> figures/appen-7.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.6\linewidth]{img/SemAcEm-plot-claude-2}
  \caption{Evaluation of different metrics on NQ dev subsets (1752 instances). SeEM is an adjusted version of EM where semantically equivalent answers are corrected via LLM prompting. The same adjustment is also applied to AcEM and refer to SeAcEM}
  \label{fig:claude-sem-equi}
\end{figure}
